SN 2020zbf: A fast-rising hydrogen-poor superluminous supernova with strong carbon lines

SN\,2020zbf is a hydrogen-poor superluminous supernova (SLSN) at $z = 0.1947$ that shows conspicuous \ion{C}{II} features at early times, in contrast to the majority of H-poor SLSNe. Its peak magnitude is $M_{\rm g}$ = $-21.2$~mag and its rise time ($\lesssim 26.4$ days from first light) places SN\,2020zbf among the fastest rising type I SLSNe. We used spectra taken from ultraviolet (UV) to near-infrared wavelengths to identify spectral features. We paid particular attention to the \ion{C}{II} lines as they present distinctive characteristics when compared to other events. We also analyzed UV and optical photometric data and modeled the light curves considering three different powering mechanisms: radioactive decay of $^{56}$Ni, magnetar spin-down, and circumstellar medium (CSM) interaction. The spectra of SN\,2020zbf match the model spectra of a C-rich low-mass magnetar-powered supernova model well. This is consistent with our light curve modeling, which supports a magnetar-powered event with an ejecta mass $M_{\rm ej}$ = 1.5~$\rm M_\odot$. However, we cannot discard the CSM-interaction model as it may also reproduce the observed features. The interaction with H-poor, carbon-oxygen CSM near peak light could explain the presence of \ion{C}{II} emission lines. A short plateau in the light curve around 35 -- 45 days after peak, in combination with the presence of an emission line at 6580~\AA,\ can also be interpreted as being due to a late interaction with an extended H-rich CSM. Both the magnetar and CSM-interaction models of SN\,2020zbf indicate that the progenitor mass at the time of explosion is between 2 and 5~$\rm M_\odot$. Modeling the spectral energy distribution of the host galaxy reveals a host mass of 10$^{8.7}$~$\rm M_\odot$, a star formation rate of 0.24$^{+0.41}_{-0.12}$~$\rm M_\odot$~yr$^{-1}$, and a metallicity of $\sim$ 0.4~$\rm Z_\odot$.

==> tab_hostcat.tex <==
\begin{table}
\caption{Host photometry}\label{tab:host_phot}
\begin{tabular}{cc}
\centering
\toprule
Instrument/Filter & Brightness\\
                  & (mag)\\
\midrule
LS/$g$        &$ 22.58  \pm 0.03$\\
LS/$r$        &$ 22.02  \pm 0.03$\\
LS/$i$        &$ 21.85  \pm 0.05$\\
LS/$z$        &$ 21.69  \pm 0.06$\\
DES/$y$       &$ 21.60  \pm 0.24$\\
\bottomrule
\end{tabular}
\tablefoot{All magnitudes are reported in the AB system and are not corrected for reddening.}
\end{table}

